HyperFLINT: Hypernetwork-based Flow Estimation and Temporal Interpolation for Scientific Ensemble Visualization

We present HyperFLINT (Hypernetwork-based FLow estimation and temporal INTerpolation), a novel deep learning-based approach for estimating flow fields, temporally interpolating scalar fields, and facilitating parameter space exploration in spatio-temporal scientific ensemble data. This work addresses the critical need to explicitly incorporate ensemble parameters into the learning process, as traditional methods often neglect these, limiting their ability to adapt to diverse simulation settings and provide meaningful insights into the data dynamics. HyperFLINT introduces a hypernetwork to account for simulation parameters, enabling it to generate accurate interpolations and flow fields for each timestep by dynamically adapting to varying conditions, thereby outperforming existing parameter-agnostic approaches. The architecture features modular neural blocks with convolutional and deconvolutional layers, supported by a hypernetwork that generates weights for the main network, allowing the model to better capture intricate simulation dynamics. A series of experiments demonstrates HyperFLINT's significantly improved performance in flow field estimation and temporal interpolation, as well as its potential in enabling parameter space exploration, offering valuable insights into complex scientific ensembles.

==> HyperFLINT_arch.tex <==
% \acronym architecture and loss
\begin{figure*}[t]
  \begin{adjustbox}{raise=4.65cm}
    \begin{minipage}[b]{0.15\textwidth}
      \centering
      \begin{tikzpicture}[>=stealth,font=\sffamily]
        % Define block styles
        \tikzstyle{input} = [rectangle, draw, fill=blue!30, text
        width=5em, text centered, minimum height=2.5em]
					
        \node (input1) [input] {$D_s$, $D_{u}$, $t$};
					
        \draw [->, line width=1.2pt] (1.1, -0.0) -- (1.8, -0.0);
					
      \end{tikzpicture}
    \end{minipage}
  \end{adjustbox}
  % }
	%
  \setlength{\fboxrule}{4pt}
  % \fcolorbox{orange!60}{white}{%
  \begin{tikzpicture}
    \node[draw, orange!60, fill=white, rounded corners, inner sep=4pt,
    line width=3pt, text=black] at (0,0) {

      \begin{minipage}[t]{0.88\textwidth} % Block
  \begin{adjustbox}{rotate=90}
    \color{black} \centering
  %		\raggedright
    \tikzstyle{convlayer} = [rectangle, rounded corners, minimum width=3.5cm, minimum height=0.55cm,text centered, draw=black, fill=Emerald!50]
    \tikzstyle{warp} = [rectangle, rounded corners, minimum width=2.0cm, minimum height=0.55cm,text centered, draw=black]
    \tikzstyle{concat} = [ellipse, minimum width=0.5cm, minimum height=0.55cm,text centered, draw=black, fill=green!20]
    \tikzstyle{arrow} = [thick,->,>=stealth]
    % \resizebox{0.48\textwidth}{!}{%
    \begin{tikzpicture}[node distance=0.45cm]
      % Define nodes
      \node (input) [draw, fill=gray!20, minimum width=1cm, minimum height=0.5cm, yshift=0.5cm, font=\footnotesize] {$\Fts{i-1}, \Ftu{i-1}, M^{i-1}, D_s, D_{u}, t$};
      \node (warp) [warp, below of=input, yshift=-0.4cm, fill=orange!60, font=\footnotesize] {Warping};
        \node [below right of=warp, font=\scriptsize, xshift=0.3cm, yshift=-0.15cm] {$\Dts{i-1}, \Dtu{i-1}$};
      \node (sum0) [concat, below of=warp, yshift=-0.5cm, fill=yellow!40, inner sep=0.1cm, font=\footnotesize] {Concat};
      \draw [arrow] (input.east) -- ++(0.4,0) |- (sum0.east);
\node (conv1) [convlayer, below of=sum0, yshift=-0.4cm, draw=red!60, very thick, minimum width=3.2cm, font=\scriptsize,
    shading=axis, shading angle=90, left color=Green!80, right color=red!20] {2$\times$\footnotesize{Conv3D}\scriptsize, st.=2};
    \node (conv2) [convlayer, below of=conv1, yshift=-0.4cm, draw=red!60, very thick, minimum width=2.6cm, font=\scriptsize, shading=axis, shading angle=90, left color=Emerald!80, right color=red!20] {3$\times$\footnotesize{Conv3D}\scriptsize, st.=1};
       \node (conv3) [convlayer, below of=conv2, yshift=-0.4cm, minimum width=2.6cm, fill=Green!80, font=\scriptsize] {\footnotesize{Conv3D}\scriptsize, st.=2}; % 1$\times$
       \node (conv4) [convlayer, below of=conv3, yshift=-0.4cm, minimum width=2.0cm, font=\scriptsize] {3$\times$\footnotesize{Conv3D}\scriptsize, st.=1};
        \node (conv5) [convlayer, below of=conv4, yshift=-0.4cm, minimum width=2.0cm, fill=violet!20, font=\scriptsize] {\footnotesize{Deconv3D}\scriptsize, st.=2}; % 1$\times$
        \node (conv6) [convlayer, below of=conv5, yshift=-0.4cm, minimum width=2.6cm, font=\scriptsize] {3$\times$\footnotesize{Conv3D}\scriptsize, st.=1};
	\node (sum2) [draw, circle, below of=conv6, yshift=-0.3cm, fill=yellow!40, inner sep=0.1cm, font=\scriptsize] {+};
	\node (conv7) [convlayer, below of=sum2, yshift=-0.3cm, minimum width=2.6cm, fill=violet!20, font=\scriptsize] {2$\times$\footnotesize{Deconv3D}\scriptsize, st.=2};
	\node (output) [draw, below of=conv7, fill=gray!20, minimum width=1cm, minimum height=0.5cm, yshift=-0.5cm, font=\footnotesize] {$\Fts{i}, \Ftu{i}, M^{i}$};
							
							% Draw edges
							\draw [arrow] (input) -- (warp);
							\draw [arrow] (warp) -- (sum0);
							\draw [arrow] (sum0) -- (conv1);
							\draw [arrow] (conv1) -- (conv2);
                                \draw [arrow] (conv2) -- (conv3);
                                \draw [arrow] (conv3) -- (conv4);
                                \draw [arrow] (conv4) -- (conv5);
                                \draw [arrow] (conv5) -- (conv6);
							\draw [arrow] (conv6) -- (sum2);
							\draw [arrow] (sum2) -- (conv7);
							\draw [arrow] (conv7) -- (output);
							\draw [arrow] (conv1.east) -- ++(0.4,0) |- (sum2.east);

							\draw[dashed, rounded corners=20pt] (-2.35,-9.4) rectangle (2.35,1.05);
						\end{tikzpicture}%
						%}
  \end{adjustbox}
\end{minipage}


\begin{minipage}[b]{0.58\textwidth} %
  \begin{adjustbox}{rotate=90}
    \tikzstyle{convblock} = [rectangle, rounded corners, minimum
    width=2.5cm, minimum height=0.9cm,text centered, draw=black,
    fill=green!40] \tikzstyle{arrow} = [thick,->,>=stealth]
    \begin{tikzpicture}[node distance=0.5cm]
      % Define nodes
      \node (input) [draw, fill=gray!20, minimum width=1.0cm, minimum height=0.7cm] {$D_s$, $D_{u}$, $t$};
      \node (conv0) [convblock, below of=input, yshift=-0.7cm] {Conv Block$^0$};
      \node (sum0) [draw, circle, below of=conv0, yshift=-0.5cm, fill=yellow!40, inner sep=0.1cm] {{+}};
      \node [above right of=sum0, font=\scriptsize, xshift=0.55cm, yshift=-0.05cm] {$\Fts{0}, \Ftu{0}, M^{0}$};
      \node (conv1) [convblock, below of=sum0, yshift=-0.5cm] {Conv Block$^1$};
      \node (sum1) [draw, circle, below of=conv1, yshift=-0.5cm, fill=yellow!40, inner sep=0.1cm] {{+}};
      \node [above right of=sum1, font=\scriptsize, xshift=0.55cm, yshift=-0.05cm] {$\Fts{1}, \Ftu{1}, M^{1}$};
      \node (conv2) [convblock, below of=sum1, yshift=-0.5cm] {Conv Block$^{2}$};
      \node (output) [draw, below of=conv2, fill=gray!20, minimum width=1cm, minimum height=0.7cm, yshift=-0.7cm] {\color{red}$\Ftu{2}, M$};
      
      % Draw edges
      \draw [arrow] (input) -- (conv0);
      \draw [arrow] (conv0) -- (sum0);
      \draw [arrow] (sum0) -- (conv1);
      \draw [arrow] (conv1) -- (sum1);
      \draw [arrow] (sum1) -- (conv2);

      \draw [arrow] (conv2) -- (output);
      \draw [arrow] (input.west) -- ++(-1.2,0) |- (sum0.west);
      \draw [arrow] (input.west) -- ++(-1.2,0) |- (sum1.west);
      \draw [arrow] (input.west) -- ++(-1.2,0) |- (sum0.west);
      \draw [arrow] (conv0.east) -- ++(0.8,0) |- (sum1.east);

      \draw [thick, dashed] (conv1.north east) -- (3.1, 1.5);
      \draw [thick, dashed] (conv1.south east) -- (3.1, -7.5);
    \end{tikzpicture}
  \end{adjustbox}
\end{minipage}

  
  % \hfill
  % \hspace{0.1\textwidth}
  % \iffalse

\begin{minipage}[b]{0.21\textwidth} % Loss
				\begin{adjustbox}{raise=0.3cm}
					
                    \color{black}
						\centering
						%	\vspace{1em}
						\begin{tikzpicture}[>=stealth,font=\sffamily]
							% Define block styles
							\tikzstyle{loss1} = [rectangle, draw, fill=cyan!40, text width=5em, text centered, minimum height=2.5em]
                                \tikzstyle{arrow} = [thick,->,>=stealth]
							% Place nodes
							\node [text=black, above] at (0,0.75) {\small\textbf{Loss function $\Loss$}};
							\node [loss1] (loss1) {$\mathcal{L}_{rec}$};
							\node [below=0.2cm of loss1, font=\Large] {+};
							
							\node [loss1, below=1cm of loss1] (loss2) {$\mathcal{L}_{flow}$};

                                \draw [arrow] (loss1.west -| {-2.4cm,0}) -- node[midway, above] {$\Dhat_{t}, {\DGT}$}  (loss1.west);
                                 
                               \draw [arrow] (loss2.west -| {-2.5cm,0}) -- node[midway, above] {$\Ft{i}, {\FGT}$}  (loss2.west);
							
						\end{tikzpicture}
  \end{adjustbox}
\end{minipage}
			% }
       };

\end{tikzpicture}
			%}
		% Manually place the text above the figure
		\begin{picture}(0,0)
			\put(-85, 290){\textbf{\normalsize{FLINT* Network}}}
		\end{picture}

\begin{tikzpicture}[remember picture, overlay]
    % Approximate the coordinates between the two figures
    \draw[dashed, ->, line width=1.2pt, color=blue] 
        (17.05, 5.25) -- (17.55, 5.25) -- (17.55, 13.35) -- (15.8, 13.35); % Adjust these coordinates to fit your layout
\end{tikzpicture}
\vspace{-18pt}
% End new figure
		\caption{ \acronym network architecture
                  and pipeline during training:
                  % (see corresponding ~\autoref{fig:nn_overview} for inference): 
                  Given the
                  input fields $D_s$ and $D_{u}$, and their simulation parameters,
                  % and $\FGT$ (GT flow at time $t$), 
                  \acronym predicts the $\hat{D}_{t}$ scalar field
                  and $\hat{F}^{i}_{t}$ flow fields used in the loss
                    function for optimizing network parameters.  
                    The \acronym model consists of two key components: the HyperNet and the main network, FLINT*. 
                    The HyperNet, depicted within the red box, generates weights for the convolutional layers of FLINT* (with red outlines in the middle column of the orange box).
                    The FLINT* model architecture and loss function are shown in the orange box.  
                    The model consists of several stacked blocks of the
                  convolutional network, which takes $D_s$, $D_{u}$,
                  and $t$ as input and in the $i^{th}$ $\cb{}$ computes
                    estimated flows $\Fts{i}, \Ftu{i}$, and fusion
                    mask $M^i$ used for interpolation.  
                    % We obtain the best results with three ($N=3$) blocks.
                  The zoomed-in view on the right highlights the structure of a generic Conv Block
                  consisting of backward warping,
                  concatenation, as well as convolutional and
                  deconvolutional layers with specified strides
                  ($st.$). The loss function, is shown on the right
                  within the orange box. The GT density $\DGT$ and flow $\FGT$ is only used in the loss function $\Lflow$.
                  The blue dashed arrow in the right of the figure represents the gradient propagation during training, from the output of FLINT* back to the HyperNet. 
                    }
		\label{fig:model}
        \vspace{-12pt}
\end{figure*}
